Differentially Private Range Query on Shortest Paths

We consider differentially private range queries on a graph where query ranges are defined as the set of edges on a shortest path of the graph. Edges in the graph carry sensitive attributes and the goal is to report the sum of these attributes on a shortest path for counting query or the minimum of the attributes in a bottleneck query. We use differential privacy to ensure that the release of these query answers provide protection of the privacy of the sensitive edge attributes. Our goal is to develop mechanisms that minimize the additive error of the reported answers with the given privacy budget. In this paper we report non-trivial results for private range queries on shortest paths. For counting range queries we can achieve an additive error of $\tilde O(n^{1/3})$ for $\varepsilon$-DP and $\tilde O(n^{1/4})$ for $(\varepsilon, \delta)$-DP. We present two algorithms where we control the final error by carefully balancing perturbation added to the edge attributes directly versus perturbation added to a subset of range query answers (which can be used for other range queries). Bottleneck range queries are easier and can be answered with polylogarithmic additive errors using standard techniques.

==> figs/GapCycle_fig.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.9, xscale=0.9, every node/.style={scale=0.9}]
%uncomment if require: \path (0,387); %set diagram left start at 0, and has height of 387

%Shape: Ellipse [id:dp5593365541387805] 
\draw   (47,200.7) .. controls (47,193.91) and (52.44,188.4) .. (59.14,188.4) .. controls (65.85,188.4) and (71.29,193.91) .. (71.29,200.7) .. controls (71.29,207.49) and (65.85,213) .. (59.14,213) .. controls (52.44,213) and (47,207.49) .. (47,200.7) -- cycle ;
%Straight Lines [id:da5146902576540848] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (445.43,301.38) -- (384,300) ;
%Straight Lines [id:da04862258291422261] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (446,358) -- (384.42,357) ;
%Straight Lines [id:da24149871316704208] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (445.43,328.38) -- (384,327) ;
%Shape: Ellipse [id:dp8146700609923305] 
\draw   (47,157.3) .. controls (47,150.51) and (52.44,145) .. (59.14,145) .. controls (65.85,145) and (71.29,150.51) .. (71.29,157.3) .. controls (71.29,164.09) and (65.85,169.6) .. (59.14,169.6) .. controls (52.44,169.6) and (47,164.09) .. (47,157.3) -- cycle ;
%Shape: Ellipse [id:dp42925657231850134] 
\draw   (118.43,200.7) .. controls (118.43,193.91) and (123.87,188.4) .. (130.57,188.4) .. controls (137.28,188.4) and (142.71,193.91) .. (142.71,200.7) .. controls (142.71,207.49) and (137.28,213) .. (130.57,213) .. controls (123.87,213) and (118.43,207.49) .. (118.43,200.7) -- cycle ;
%Shape: Ellipse [id:dp48695029032586823] 
\draw   (118.43,157.3) .. controls (118.43,150.51) and (123.87,145) .. (130.57,145) .. controls (137.28,145) and (142.71,150.51) .. (142.71,157.3) .. controls (142.71,164.09) and (137.28,169.6) .. (130.57,169.6) .. controls (123.87,169.6) and (118.43,164.09) .. (118.43,157.3) -- cycle ;
%Shape: Ellipse [id:dp41781531392704996] 
\draw   (347,200.7) .. controls (347,193.91) and (352.44,188.4) .. (359.14,188.4) .. controls (365.85,188.4) and (371.29,193.91) .. (371.29,200.7) .. controls (371.29,207.49) and (365.85,213) .. (359.14,213) .. controls (352.44,213) and (347,207.49) .. (347,200.7) -- cycle ;
%Shape: Ellipse [id:dp6866360225027914] 
\draw   (347,157.3) .. controls (347,150.51) and (352.44,145) .. (359.14,145) .. controls (365.85,145) and (371.29,150.51) .. (371.29,157.3) .. controls (371.29,164.09) and (365.85,169.6) .. (359.14,169.6) .. controls (352.44,169.6) and (347,164.09) .. (347,157.3) -- cycle ;
%Shape: Ellipse [id:dp17175244482681107] 
\draw   (418.43,200.7) .. controls (418.43,193.91) and (423.87,188.4) .. (430.57,188.4) .. controls (437.28,188.4) and (442.71,193.91) .. (442.71,200.7) .. controls (442.71,207.49) and (437.28,213) .. (430.57,213) .. controls (423.87,213) and (418.43,207.49) .. (418.43,200.7) -- cycle ;
%Shape: Ellipse [id:dp5980794565610463] 
\draw   (418.43,157.3) .. controls (418.43,150.51) and (423.87,145) .. (430.57,145) .. controls (437.28,145) and (442.71,150.51) .. (442.71,157.3) .. controls (442.71,164.09) and (437.28,169.6) .. (430.57,169.6) .. controls (423.87,169.6) and (418.43,164.09) .. (418.43,157.3) -- cycle ;
%Shape: Ellipse [id:dp930346203604349] 
\draw   (197,90.7) .. controls (197,83.91) and (202.44,78.4) .. (209.14,78.4) .. controls (215.85,78.4) and (221.29,83.91) .. (221.29,90.7) .. controls (221.29,97.49) and (215.85,103) .. (209.14,103) .. controls (202.44,103) and (197,97.49) .. (197,90.7) -- cycle ;
%Shape: Ellipse [id:dp5152529348948689] 
\draw   (197,47.3) .. controls (197,40.51) and (202.44,35) .. (209.14,35) .. controls (215.85,35) and (221.29,40.51) .. (221.29,47.3) .. controls (221.29,54.09) and (215.85,59.6) .. (209.14,59.6) .. controls (202.44,59.6) and (197,54.09) .. (197,47.3) -- cycle ;
%Shape: Ellipse [id:dp4044787931623841] 
\draw   (268.43,90.7) .. controls (268.43,83.91) and (273.87,78.4) .. (280.57,78.4) .. controls (287.28,78.4) and (292.71,83.91) .. (292.71,90.7) .. controls (292.71,97.49) and (287.28,103) .. (280.57,103) .. controls (273.87,103) and (268.43,97.49) .. (268.43,90.7) -- cycle ;
%Shape: Ellipse [id:dp1856556888290184] 
\draw   (268.43,47.3) .. controls (268.43,40.51) and (273.87,35) .. (280.57,35) .. controls (287.28,35) and (292.71,40.51) .. (292.71,47.3) .. controls (292.71,54.09) and (287.28,59.6) .. (280.57,59.6) .. controls (273.87,59.6) and (268.43,54.09) .. (268.43,47.3) -- cycle ;
%Shape: Ellipse [id:dp01511114581209605] 
\draw   (227,320.7) .. controls (227,313.91) and (232.44,308.4) .. (239.14,308.4) .. controls (245.85,308.4) and (251.29,313.91) .. (251.29,320.7) .. controls (251.29,327.49) and (245.85,333) .. (239.14,333) .. controls (232.44,333) and (227,327.49) .. (227,320.7) -- cycle ;
%Shape: Ellipse [id:dp21991271907689924] 
\draw   (228.43,280.7) .. controls (228.43,273.91) and (233.87,268.4) .. (240.57,268.4) .. controls (247.28,268.4) and (252.71,273.91) .. (252.71,280.7) .. controls (252.71,287.49) and (247.28,293) .. (240.57,293) .. controls (233.87,293) and (228.43,287.49) .. (228.43,280.7) -- cycle ;
%Straight Lines [id:da1965775089312216] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (59.14,169.6) -- (59.14,188.4) ;
%Straight Lines [id:da24806850452919194] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (130.57,169.6) -- (130.57,188.4) ;
%Straight Lines [id:da6975635703890408] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (268.43,47.3) -- (221.29,47.3) ;
%Straight Lines [id:da7780569578007075] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (268.43,90.7) -- (221.29,90.7) ;
%Straight Lines [id:da4057139240138756] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (359.14,188.4) -- (430.57,169.6) ;
%Straight Lines [id:da6301596283167199] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (430.57,188.4) -- (359.14,169.6) ;
%Straight Lines [id:da24355304941799116] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (197,47.3) -- (59.14,145) ;
%Straight Lines [id:da06004447404137547] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (197,90.7) -- (130.57,145) ;
%Straight Lines [id:da890973511478738] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (292.71,47.3) -- (430.57,145) ;
%Straight Lines [id:da17122712651407834] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (292.71,90.7) -- (359.14,145) ;
%Straight Lines [id:da4892019054558363] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (252.71,280.7) -- (352,210) ;
%Straight Lines [id:da6821102149872449] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (251.29,320.7) -- (430.57,213) ;
%Straight Lines [id:da39946689273877145] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (228.43,280.7) -- (130.57,213) ;
%Straight Lines [id:da02086555149591307] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (59.14,213) -- (227,320.7) ;

% Text Node
\draw (75.14,203.81) node [anchor=north west][inner sep=0.75pt]    {$u_{1}$};
% Text Node
\draw (383,255) node [anchor=north west][inner sep=0.75pt]    {$t=3$};
% Text Node
\draw (151.57,206.02) node [anchor=north west][inner sep=0.75pt]    {$u'_{1}$};
% Text Node
\draw (460,288) node [anchor=north west][inner sep=0.75pt]   [align=left] {Edges of Alice \ $\displaystyle x_{i} =0$};
% Text Node
\draw (460,346) node [anchor=north west][inner sep=0.75pt]   [align=left] {Edges of Bob};
% Text Node
\draw (460,315) node [anchor=north west][inner sep=0.75pt]   [align=left] {Edges of Alice \ $\displaystyle x_{i} =1$};
% Text Node
\draw (74.57,161.81) node [anchor=north west][inner sep=0.75pt]    {$v_{1}$};
% Text Node
\draw (148,164.02) node [anchor=north west][inner sep=0.75pt]    {$v'_{1}$};
% Text Node
\draw (374.14,207.81) node [anchor=north west][inner sep=0.75pt]    {$v'_{3}$};
% Text Node
\draw (449.57,196.02) node [anchor=north west][inner sep=0.75pt]    {$v_{3}$};
% Text Node
\draw (374.57,153.81) node [anchor=north west][inner sep=0.75pt]    {$u'_{3}$};
% Text Node
\draw (448,153.02) node [anchor=north west][inner sep=0.75pt]    {$u_{3}$};
% Text Node
\draw (303.14,42.81) node [anchor=north west][inner sep=0.75pt]    {$v_{2}$};
% Text Node
\draw (226.57,36.02) node [anchor=north west][inner sep=0.75pt]    {$u_{2}$};
% Text Node
\draw (296.57,83.81) node [anchor=north west][inner sep=0.75pt]    {$v'_{2}$};
% Text Node
\draw (224,91.02) node [anchor=north west][inner sep=0.75pt]    {$u'_{2}$};
% Text Node
\draw (256.57,281.81) node [anchor=north west][inner sep=0.75pt]    {$\tilde{u}_{j}$};
% Text Node
\draw (256.57,326.81) node [anchor=north west][inner sep=0.75pt]    {$\tilde{u}_{j}$};

\end{tikzpicture}




==> range-query.tex <==
% \subsection{Shortest Paths as Ranges}
% \label{subsec:range-query-sp}
%Jie: just to put down references and a sketch.

In a set system $\R=(X, \S)$, $X$ is a set of elements and $\S$ is a collection of subsets $S_i\subseteq X$ called \emph{ranges}. In a graph $G$ when shortest paths are unique\footnote{One can use symbolic perturbation of edge weights to produce unique shortest paths.}, we can define shortest paths as ranges.
We take $X$ to be the set of $n$ vertices and each set of $\S$ corresponds to the set of vertices on a shortest path. When $G$ is undirected, $\S$ has ${n \choose 2}$ sets. When $G$ is directed, $\S$ may have up to $n^2$ sets. % \chen{expand this}




